Intuitions of Compromise: Utilitarianism vs. Contractualism

What is the best compromise in a situation where different people value different things? The most commonly accepted method for answering this question -- in fields across the behavioral and social sciences, decision theory, philosophy, and artificial intelligence development -- is simply to add up utilities associated with the different options and pick the solution with the largest sum. This ``utilitarian'' approach seems like the obvious, theory-neutral way of approaching the problem. But there is an important, though often-ignored, alternative: a ``contractualist'' approach, which advocates for an agreement-driven method of deciding. Remarkably, no research has presented empirical evidence directly comparing the intuitive plausibility of these two approaches. In this paper, we systematically explore the proposals suggested by each algorithm (the ``Utilitarian Sum'' and the contractualist ''Nash Product''), using a paradigm that applies those algorithms to aggregating preferences across groups in a social decision-making context. While the dominant approach to value aggregation up to now has been utilitarian, we find that people strongly prefer the aggregations recommended by the contractualist algorithm. Finally, we compare the judgments of large language models (LLMs) to that of our (human) participants, finding important misalignment between model and human preferences.

==> sections/old_introduction_and_related_work.tex <==
%% everything that was in the (1) introduction and (2) related work sections on April 5, 2024 was copied to here.


\iftoggle{pnas}{
    \dropcap{Y}ou
}{
    You
}         
lead a diverse grant-making body answerable to constituents with competing views.  Whom should you fund? You might allocate funds in proportion to the size of constituents and their need---this could result in making things better in expectation. You might call the constituents together to discuss the issue---this could result in determining what all the invested parties would agree to.
As you run through these possibilities, you aren't simply uncertain about what to do, you're uncertain about \textit{how to decide} what to do.  Is this a situation that calls for  maximizing expected utility, achieving consensus, or something else?  Different values call for different solutions to the problem.
% Imagine you find a diamond ring on the floor of a crowded restaurant.  What should you do with it?  You might first think to try to return it to the (likely distraught) ringless patron---surely the right thing to do is to respect the property rights of the ring's owner.  After a moment's reflection, however, other possibilities may jump to mind.  You could sell the ring and donate the money to charity---this could result in making things better for the world's worst off people.  You could call all the diners to attention and discuss the issue---this could result in determining what all the invested parties would agree to. You could pocket the ring and go on with your day---this would certainly be the easiest thing to do and would be the best outcome for you.

% If you care about each one, is there a way to figure out what to do that combines them all?

This is the widely studied puzzle of value aggregation.
% A city council must decide how to use tax revenue.  Whose interests get priority?
% We are constantly faced with the question of how to aggregate perspectives, views, preferences, and values--and the more you look, the more it becomes apparent that this issue pervades our personal and communal lives. 
At the core of each of these questions is the problem of how we ought to aggregate views. This arises in how to construct democratic voting systems, what definition of fairness to use, and how to define behavior for rational agents. 

% You sit down for dinner pining for a burger but torn up about animal welfare. What should you eat? 


\jared{Fiery: condense the above three paragraphs into one}

Given the centrality of this question to issues in rational decision-theory, social choice, and constructing democratic voting systems, you might expect there to be a rich literature formalizing proposals for how to deal with value aggregation and then testing those proposals against people's intuitions. However, to our knowledge, insufficient prior work has directly compared people’s intuitions of two of the most obvious candidates for how aggregation should work--taking the \textit{sum} of all the values (the classic ``utilitarian'' approach, Equation~\ref{equation-sum}) and the \textit{product} (a less well-known ``contractualist'' approach, Equation~\ref{equation-product}).
\jared{Yejin suggests "little prior work" instead of "no prior work". This also seems to be where we would make salient the comparison with prior work on MEC, NBS. Not sure how to make it more salient than this sentence except by italicizing, e.g.}
\jared{Fiery agrees. "Rather than saying nobody has ever studied anything like this, maybe you can instead briefly (and approvingly) summarize what people HAVE studied that is SIMILAR, and then give a more robust defense of why your particular innovations are a key advance.  (Because you consider a product rule?  Because you test against human intuitions?  Both?)"}
\jared{Bailey: When utilities can be near zero (which I'm assuming they can here?), from a mathematical perspective, the geometric mean acts very much like maximin egalitarianism (i.e, making the worst-off person as well-off as possible), because the geometric mean is very sensitive to low values (think about if a single utility approaches 0 and all others are fairly close to 1 --- the product will be close to 0). Not sure if you need to say this here exactly, but this may be useful intuition.}

\jared{Fiery wants more of the related work in the introduction. "You’re taking the existing literature seriously, and you’re being concrete.  I would love to see elements of this reflected in the introduction"}

 % However, to our knowledge, there exists no formal model of moral uncertainty that has also been empirically verified. 

% Philosophers call this puzzle ``moral uncertainty'' and the more you look, the more it becomes apparent that this issue pervades our personal and communal lives \citep{macaskill_normative_2016}. You sit down for dinner pining for a burger but torn up about animal welfare. How do you decide what to eat?  A diverse grant-making body is answerable to constituents with competing views.  How does it decide who to fund?  A city council must decide how to use tax revenue.  How do they decide whose interests get priority?

% These issues become even more thorny when AI systems are involved. Existing AI systems already make morally-charged decisions. From deciding whose content should be shown first on a feed, to who gets to have an interview given their resumes, to which route to recommend (the shortest, the most environmentally friendly, the safest?) there are many examples of existing systems which implicitly operate in a moral setting. Different moral theories would make different recommendations about how to answer moral questions that arise for these systems.  And if you ask different people how to resolve these dilemmas, they may provide different answers that are produced by different methods of decision-making.  Without even realizing it, system designers end up committing not just to specific \textit{normative} accounts---i.e., accounts that dictate what the right thing to do is---but often also to to specific \textit{meta-normative} accounts---i.e., accounts about how to resolve uncertainty over the correct normative account.

%\subsection*{Contributions}
In this work, we empirically survey participants' intuitions about the recommendations given by the leading formal algorithms for aggregating value. Unlike most past work, we randomly generate and sample the proposals suggested by each algorithm instead of looking at isolated, illustrative cases. In addition, we design a series of visual aids to convey the proposals to participants.  This allows us to use quantitatively precise stimuli, while not overwhelming subjects with task-intensive, numerical comparisons.  
Finally, we compare the judgments of large language models (LLMs) to that of our (human) participants, finding marked differences between and across model sizes. Both empirical data \citep{bruner_decisions_2018, frohlich_laboratory_1987}
and dominant assumptions in fields from decision theory, to AI, to philosophy have favored a utilitarian approach to value aggregation. Despite this, we know of no empirical work that has directly compared utilitarian and contractualist aggregation mechanisms. On the contrary, we find that both humans and performant LLMs prefer an agreement-based, contractualist approach which involves taking a \textit{product} of values, not a \textit{sum}.



%%%%%%%%%%%%%%%%%
%%%%% old related work section
%%%%%%%%%%%%%%%%%%%

%\section*{Related Work}
%\label{sec:related-work}

% January, 2024: Removed this comment
% \sydney{Big question: I re-framed the intro to target a larger audience, but getting clear on our audience will impact what should fall into related work.  Right now, my sense is that this section speaks to philosophers and AI researchers.  But I think we can pitch this more broadly -- ie, to people working in rational decision-theory, social choice, and voting theory--and that will be especially important if we want to submit to PNAS.  But to make those claims, the related work section should canvas attempts at formalizing preference aggregation across those fields.  Does this seem doable?}
% \jared{I may not have time for this soon.}

% \subsection*{Aggregating Human Preferences}


\jared{Bailey: When utilities can be near zero (which I'm assuming they can here?), from a mathematical perspective, the geometric mean acts very much like maximin egalitarianism (i.e, making the worst-off person as well-off as possible), because the geometric mean is very sensitive to low values (think about if a single utility approaches 0 and all others are fairly close to 1 --- the product will be close to 0). Not sure if you need to say this here exactly, but this may be useful intuition.}

\subsection*{Theoretical Foundations}

The literature on aggregating human preferences spans rational decision-theory \citep{von_neumann_theory_1947, luce_games_1957, tversky_intransitivity_1969}, social choice theory \citep{sen_collective_2018}, and voting theory \citep{riker_theory_1968}. These theoretical frameworks offer distinct perspectives on how individual preferences can be consolidated into collective decisions.

Rational decision-theory, as the basis of understanding individual preferences, posits that individuals, when faced with multiple options, will choose the one that maximizes their utility \citep{von_neumann_theory_1947}.
This implies that preferences are transitive and consistent \citep{luce_games_1957}. However, when multiple individual preferences are aggregated, these assumptions may not hold, leading to a variety of paradoxes \citep{arrow_difficulty_1950, tversky_intransitivity_1969, kahneman_prospect_2013, samuelson_note_1938}.
% such as Arrow's impossibility theorem \citep{arrow_difficulty_1950}, the intransitivity of preferences \citep{tversky_intransitivity_1969, kahneman_prospect_2013}, or the difference between revealed and expressed preferences \citep{samuelson_note_1938}.

Social choice theory, as an extension of rational decision-theory, analyzes individual preferences in a society and how they can be aggregated to reflect a collective preference \citep{sen_collective_2018}. It focuses on the design of mechanisms for making collective decisions, namely social welfare functions (SWFs). SWFs rank decisions based on their desirability to some group. Here we will exclusively be looking at cardinal SWFs, those which assume a numeric utility (outcome) for various groups.
% Still, social choice theory often assumes that individual preferences are fixed and does not consider the potential for preference change over time \citep{brock_discrete_2001}.
Voting theory overlaps with social choice theory and specifically addresses the methodology of preference aggregation in democratic decision-making processes \citep{riker_theory_1968}.
Defining utilities carries large assumptions. For example, in economics, one might simply use a fungible price as a utility while utilities of outcomes in voting theory are not fungible. Furthermore, people may use different value functions to make decisions. In our experiments, we included both non-fungible and fungible quantities (see sec. "Study 1").
%Usually, voting functions assume less about the preferences over which they operate. For example, the majority vote suffices with binary classification as opposed to cardinal outcomes \citep{black_theory_1958}. Unique to voting theory are concerns over representation and sampling, and strategic manipulation \citep{gibbard_manipulation_1973, satterthwaite_strategy-proofness_1975}, which we  avoid in our work by asking participants to evaluate given examples.
%\jared{could cut the above paragraph entirely}

\jared{Bailey: Depending on what utilities mean in the context, people may use different value functions to make decisions. I think in your study, it is important to make these distinctions clearly and state which interpretation(s) you think are relevant to your experimental setup.}

\jared{Fiery: "Also, I’m lost in the third paragraph (“Social choice theory…”) because I’m guessing that somehow this is supposed to align with “products” and with “contractualism”, but you haven’t actually made any of this explicit." That isn't what we are trying to do here so I am confused what he picked up on.}

\jared{Fiery wants us to put here "a transitional section where you establish the goals and basic design of your modeling framework in plain english?"}

% TODO: cite pluralistic alignment somewhere?

\paragraph{Definitions} Let \(A\) be the set of groups.
% (we will also call these theories or perspectives)
Let \(B\) be a set of voting power (size) for each group in the space of
\([0,1]^{|A|}\).
% (we will also call these credences)
Let \(C\) be the
set of choices (or proposals). Let \(U\) in \(\mathbb{R}^{|B|\times|A|}\) for the cardinal
case
% and \(\mathbb{N}^{|C|\times|A|}\) for the ordinal 
be the outcomes (utilities)
associated for a particular group with a choice, where a particular
choice, \(c\), and group \(a\), outcome is denoted \(u_a(c)\).

\paragraph{Aggregation Mechanisms}
There are a variety of SWFs which one might use to aggregate views. We will consider two of the most popular. Note, all aggregation mechanisms non-trivially assume known utilities.
First consider the Utilitarian social welfare function, e.g. as identified by \citet{von_neumann_theory_1947}, which we will term the "Utilitarian Sum". Formally, this \textit{sums} the utility of available choices based on the degree of support for each. 

\begin{equation}
\argmax_{c \in C} \sum_{a \in A} u_a(c) \times b_a
\label{equation-sum}
\end{equation}


\noindent There are many ways in which the Utilitarian Sum is intuitively appealing.  For instance, it uses logic similar to what we use for dealing with \emph{empirical} uncertainty in a rational actor framework---simply do the action that leads to the best consequence taking into account how likely each consequence is and how good or bad it would be \citep{buchak_risk_2013},  equating degree of likelihood and belief.
% Another strong appeal is that the view can be easily algorithmically defined.
However, the Utilitarian Sum also has important drawbacks. For instance, the Utilitarian Sum biases toward strong opinions of minority sub-groups---an issue called \textit{fanatacism}.
% For example if with two groups, $a$ and $b$, and two choices, $1$ and $2$, where $c_a = .9$, $c_b=.1$, $u_1(a) = 1$;$u_2(a)=-1$;$u_1(b) = -100$;$u_2(b)=100$, Utilitarian Sum will be swayed to the fanatical position of choosing $2$.

It also makes \textit{inter-theoretic comparisons}: direct comparisons between the utilities of different groups which is  difficult to justify \textit{a priori}. The Utilitarian Sum has been widely studied, particularly as it relates to empirical uncertainty.

In contrast, \citet{kaneko_nash_1979} introduce the Nash Social Welfare Function which we will term the "Nash Product". Formally, the solution to a Nash bargaining problem is 
% an optimization problem to find the (n-)rectangle of greatest area with vertices at the origin and on the Pareto frontier, that is to
to maximize the \textit{product} of utilities \citep{zamir_game_2013}: 

\begin{equation}
\argmax_{c \in C} \prod_{a \in A} u_a(c)^{b_a}
\label{equation-product}
\end{equation}

\noindent Because we focus on the symmetric case, when groups have the same voting power, we leave off the exponent, $b_a$.
\jared{Fiery: "Is it to maximize the products of utilities, or the product of utility gains?" Jared: I don't understand the difference.}

% Both Nash Product and Utilitarian Sum can be seen as parameterized SWFs in which the Rawlsian (lexicographic minimum), and the Utilitarian Utilitarian Sum define extremal points \citep{bakker_fine-tuning_2022}.

\paragraph{Arguing for Aggregation Mechanisms}
How do we judge whether one aggregation mechanism is superior to another?

One approach is to examine the theoretical, mathematical trade-offs between them. More recent theoretical work on the Nash Product in social welfare largely seeks to approximate it with various trade-offs \citep{mcglaughlin_improving_2020, branzei_nash_2017, ramezani_nash_2010} as opposed to compare it to other aggregation approaches, such as we do, comparing the \textit{Utilitarian Sum} and \textit{Nash Product}. Still, there have been a number of comparisons between the Nash Product and Utilitarian Sum-like approaches in terms of their mathematical character \citep{rachmilevitch_nash_2023, rachmilevitch_egalitarianism_2019, rachmilevitch_nash_2015, thomson_nashs_1981}.  Closer to our focus on moral decision making, \citet{kimbrough_meta-theory_2023} propose a number of game-theoretic heuristics (including the Nash Product) which might be used to proxy for moral choice and simulate how often those heuristics would accord with an underlying payoff vector in a variety of games.

\iftoggle{pnas}{

\figureScenarioPNAS

}{
\figureScenario
}

Another way to judge which aggregation mechanism is better entails examining isolated, edge cases and using individual intuitions about those cases as justification for one mechanism or another.
% \paragraph{Moral Uncertainty: A Case Study}
This approach to preference aggregation is quite visible in moral philosophy. \citet{macaskill_normative_2016} introduces moral uncertainty as an answer
for what to do when you believe in
different ethical theories by different amounts. Unlike when aggregating preferences across a group, the focus here is on aggregating across multiple models of behavior. Drawing on the logic of \emph{consequentialist moral philosophy} and \citet{macaskill_normative_2016, macaskill_why_2020} argue for the Utilitarian Maximum Expected Choice-worthiness (MEC). MEC is equivalent to the Utilitarian social welfare function (SWF) from social choice theory when construed as aggregating the opinions of different group members. 

% He describes My Favorite Theory (MFT) which deems the most appropriate
% choice as the choice deemed most appropriate by the theory you believe in the most.

% \begin{equation}
% \argmax_{c \in C} u_{(\argmax_{a \in A} b_a)}(c)
% \end{equation}

%for the cardinal case.
%  and Borda-count
% ranked-choice voting for the ordinal case.
% We will use the term Utilitarian Sum to
% refer to both.

% \citet{gracely_noncomparability_1996} argues that it is fundamentally invalid to compare the degrees of support (utility) which different ethical theories might use to construe the appropriateess of an action. \citet{gustafsson_defence_2014} further makes the case that the majority-vote does the best job at avoiding such intertheoretic comparisons. 
% \iftoggle{pnas}{
% Nonetheless, empirical uncertainty is not the same as disagreement. Modeling them the same way carries strong meta-ethical commitments.
% }
To the contrary, \citet{newberry_parliamentary_2021} argue for a \emph{contractualist} (or agreement-based) logic as opposed to a consequentialist one. 
% The authors argue for a ``moral parliament'' approach to resolving moral uncertainty, whereby various theories send representatives to an imaginary parliament.  A compromise results from a structured ``negotiation'' between the views. \citet{newberry_parliamentary_2021}, however, do not formalize their view leaving open a wide range of ways that a moral parliament approach could potentially be implemented.
\citet{greaves_bargaining-theoretic_2023} point out that the Nash bargaining solution (Nash Product), also called the Nash product social welfare function (SWF) captures many of the virtues of this suggestion. Nonetheless, \citet{greaves_bargaining-theoretic_2023} argue against the Nash Product in favor of the Utilitarian Sum, arguing against its \emph{conservatism}.

% To do so, they introduce a disagreement point,
% \(\mathbf{d} \in \mathbb{R}^{|A|}\) the default outcome if no negotiation is
% reached, such that the outcome of the disagreement point is also an
% available utility for each agent, \(U \cup \{ \mathbf{d} \}\).


% TODO: could talk about fanatacism, inter-theoretic comparisons, and variance normalization here, if space permits


\paragraph{Summing Up} The above approaches theoretically seek to justify one aggregation method over other, often picking single cases out as intuitive counter-examples \citep{macaskill_normative_2016, newberry_parliamentary_2021, greaves_bargaining-theoretic_2023} or axiomatically seeking the most `rational' aggregation mechanism \citep{von_neumann_theory_1947, kaneko_nash_1979}. \iftoggle{pnas}{(See SI sec. "Aggregating Preferences in AI" for how AI literature generally assumes something like the Utilitarian Sum.)}{}
Less work has sought to ground the determination of the appropriate aggregation mechanism in studies of the decisions that people actually make.  We now turn to reviewing that literature.

\subsection*{Experimental Foundations}

\jared{Fiery wants this in the introduction. "It feels disorienting to have this lit review here.  Shouldn’t this be in the introduction?  All of this feels like helpful setup I would have appreciated in the introduction."}

\paragraph*{Economic Psychology} When people make decisions between multiple outcomes, what approaches do they tend to make? Questions such as this are the domain of economic psychology. A number of works examine which resource distributions people favor, finding some evidence for fairness \citep{charness_understanding_2002, engelmann_inequality_2004, fehr_inequality_2006}.

Other work in economic psychology has homed in on the Nash Product, studying the effect of the disagreement point, the no-compromise option \citep{bruce_impact_2012}, characterizing different strategies in bargaining games \citep{kroll_bargaining_2014}, and framing it as a trade-off between utility or money \citep{berninghaus_trading_2008}.
In practice, \citet{yao_modeling_2021} find that in a certain modeling problem the Nash Product better fits the data than a Utilitarian approach, although they do not probe human intuitions directly.

\paragraph*{Empirical Philosophy}
Empirical inquiry has increasingly been used in ethical theory in attempts to validate individual philosophers’ intuitions with the opinions of the crowd, such as distributive justice \citep{frohlich_choosing_1992}, making thought-experiments real experiments (namely, Rawls’ veil of ignorance \citep{rawls_outline_1951}). \citet{bruner_decisions_2018}, for example, find that when presented with a variety of scenarios of different resource distributions, participants prefer a strictly Utilitarian approach as compared to the Rawlsian Difference Principle--participants maximize total utility not the utility for the least advantaged member. This is in line with historical results \citep{frohlich_laboratory_1987}. 

Similarly, \citet{bauer_need_2022} systematically use scenarios to
 % and gather judgements on them, 
study how various traits of agents change how much of a given resource participants distribute.
% , although they do not focus on Utilitarian Sum or Nash Product in particular.

\paragraph*{Utilitarian Sum vs. Nash Product}

We have found only one work which empirically examines participants' responses regarding the Utilitarian Sum and Nash Product. Classically, \citet{binmore_focal_1993} studied a variety of solution concepts, including the Nash Product and Utilitarian Sum, finding that it was more difficult to push participants to the Utilitarian Sum-supported answer. They ask: is human behavior more susceptible to influence by one of various aggregation mechanisms? We ask: when asked to make judgements, which aggregation mechanism best describes humans' decisions? We update \citet{binmore_focal_1993}'s work with a more direct comparison between the Utilitarian Sum and Nash Product.
\jared{Could add this to address Fiery's question about how Binmore does not pre-empt us: Specifically, \citet{binmore_focal_1993} look at the influence of "focal points", of various assumed default positions, in coordination games. Their comparison of the Utilitarian Sum and Nash Product comes in assuming that each determines the default choice assuming no agreement in a coordination game. After having subjects play 10 games biased to one focal point or another, they find that it is more difficult to move subjects toward a Utilitarian focal point than it is to a Nash Product focal point. There was no value judgement in this comparison; unlike us they did not attempt to determine which aggregation mechanism best aligned with  participants judgements of a "best compromise."}
\jared{I would almost move this work to the prior section in terms of mathematical character. I think it is confusing to mention-- yes do this, Sydney agrees}
In all, we have encountered no works which directly study whether people prefer the  the Nash Product or the 
Utilitarian Sum for value aggregation problems.  We attempt to answer that question here.

% and in the asymmetric case as so:

% \begin{equation}
% \argmax_{c \in C} \prod_{a \in A} u_a(c)^{b_a}
% \end{equation}


